Quantum integrability and functional equations

In this thesis a general procedure to represent the integral Bethe Ansatz equations in the form of the Reimann-Hilbert problem is given. This allows us to study in simple way integrable spin chains in the thermodynamic limit. Based on the functional equations we give the procedure that allows finding the subleading orders in the solution of various integral equations solved to the leading order by the Wiener-Hopf technics. The integral equations are studied in the context of the AdS/CFT correspondence, where their solution allows verification of the integrability conjecture up to two loops of the strong coupling expansion. In the context of the two-dimensional sigma models we analyze the large-order behavior of the asymptotic perturbative expansion. Obtained experience with the functional representation of the integral equations allowed us also to solve explicitly the crossing equations that appear in the AdS/CFT spectral problem.

==> susywiththook.tex <==
\chapter{\label{ch:susyspch}Supersymmetric spin chains}
%The study of integrable systems based on supersymmetric groups was initially motivated by various problems in nuclear [] and condense matter physics []. It achieved additional impetus after discovery of integrability in the AdS/CFT correspondence.
The current achievements in the field of supersymmetric integrable systems can be summarized as follows\footnote{We will restrict to the most studied case of $gl(N|M)$ algebras.}. Most of the algebraic constructions based on the $gl(N)$ algebra have a direct generalization to the supersymmetric case. However, these generalizations do not cover the all variety of properties of supersymmetric systems. Also, the physics of the excitations over the antiferromagnetic vacuum is much more complicated and was studied to some extent only for few simple cases.

Generalizing $gl(N)$ case construction, all finite-dimensional irreducible representations (irreps) of $gl(N|M)$ algebra were constructed by Kac \cite{Kac:1977em,Kac:1977qb} as highest weight representations. Equivalently these representations can be labeled by Young tableaux. The determinant Weyl formula for characters and its parameter dependent generalization - Bazhanov-Reshetikhin formula has a straightforward generalization \cite{Kazakov:2007na}. This allows, in a complete analogy with $gl(N)$ case, to construct the nested Bethe Ansatz for a supersymmetric group from Hirota dynamics via a chain of Backlund transforms \cite{Kazakov:2007fy}. The Bethe Ansatz equations can be also derived using analytical Bethe Ansatz technics \cite{Ragoucy:2007kg}.

%However, direct generalizations from the nonsupersymmetric case do not cover the all variety of properties of supersymmetric systems. This is mainly related to the fact that the structure of the representations of Lie superalgebras is richer and more complicated then those for the nonsupersymmetric case.

What makes the $gl(N|M)$ case more difficult than the $gl(N)$ case is that Lie superalgebras allow also reducible but indecomposable representations. A good example is the $sl(2|1)$ algebra representations of which were studied in \cite{Scheunert:1976wj,Marcu:1979se}.  Although all irreps of $gl(N|M)$ were classified, the complete classification of indecomposable representations for arbitrary supersymmetric simple algebra is not known\footnote{This is mainly due to the representations of zig-zag type. See \cite{Gotz:2005jz} and references therein.}.


%The irreps of superalgebras can be of two types: typical and atypical. Typical irreps enter only as a direct sum into any kind of reducible representation. Atypical irreps can be submodules of indecomposable representations. As a rule, a fundamental representation is an atypical one.

Even if we consider only irreducible representations, their tensor product may contain an indecomposable representation. It is possible to restrict to the class of the representations tensor product of which is given by a direct sum of irreps. Unfortunately, such restriction does not allow construction of a spin chain which contains a singlet state (antiferromagnetic vacuum). Therefore, whenever an antiferromagnetic vacuum is present in a spin chain, studying of excitations around this vacuum encounters the problem of presence of irreducible representations; this leads to significant complications in the construction of a physical theory \cite{Essler:2005ag,Saleur:2006tf}.

Here we aim to discuss the techniques mostly for further applications to the integrable system that appears in the context of the AdS/CFT correspondence. It turns out that, at least for the purposes of this text, it is sufficient to consider the class of irreps that do not contain indecomposable parts in their tensor product. These representations can be obtained from tensoring of the fundamental representation.

In this chapter we will first recall basic properties of the supersymmetric algebras and theirs representations on the example of the $sl(2|1)$ algebra. Then we will discuss the structure of the representations that appear as a result of the fusion procedure for the $gl(N|M)$ case. We will see that, as in the nonsupersymmetric case, the string-like solutions are in the one-to-one correspondence with rectangular irreps. The corresponding integral equations will be naturally written on a fat hook shape, or in a more general case - on a T-hook shape.

The fusion relations for a fat hook shape and a T-hook shape were discussed in \cite{Kazakov:2007fy,Hegedus:2009ky}. In the context of the AdS/CFT correspondence the T-hook shape was first proposed in \cite{Gromov:2009tv} and then in \cite{Bombardelli:2009ns,Gromov:2009bc} built starting from the string hypothesis of \cite{Takahashi:1972,Arutyunov:2009zu}. The string hypotheses and TBA systems for various cases were also known in the literature before \cite{Saleur:1999cx}.

In Sec.~\ref{sec:stringhyp} we present a general construction: the string hypothesis and corresponding functional equations for the resolvents\footnote{Equivalently, we can write integral equations for the density functions.} for $gl(N|M)$ algebra and for Bethe equations with one arbitrary source term. The Bethe equations may be based on any Kac-Dynkin diagram. Although this generalization of \cite{Takahashi:1972,Saleur:1999cx,Gromov:2009tv} is quite obvious, it was not discussed in the literature before.

 %For generic values of  $b$ we get a so called typical irrep. Such representation can enter only as a direct sum into any kind of reducible representations. However, for some discrete set of values of $b$ we get irreps that can be submodules in indecomposable representations. Such representations are called atypical or short. They are called short since their dimension is smaller then the dimension of typical irrep which is caracterized by the same Cartan weights except $b$, which is different.
%
%When we consider the tensor product of two representations with parameters $b_1$ and $b_2$, the result will be the sum of the representations with parameters $b_1+b_2-k$, where $k$ can be different for different representations in the sum. If $b_1+b_2-k$ hits mentioned discrete set of  values, the indecomposable representation may appear.
%
%Often the representation with $b_1+b_2-k\neq 0$ if $b_1>0$ and $b_2>0$. Therefore the presence of a singlet state (antiferromagnetic vacuum) in a supersymmetric spin chain is not granted. One should use for example an alternating spin chain\footnote{A chain in which odd nodes carry one representation and even nodes carry its conjugated} to attain this goal \cite{Essler:2005ag}. The other problem, which is probably related to the absence of a singlet state, is that it is not obvious what Bethe roots should be a subject of a particle-hole transformation. In fact, to write the interaction of string densities in a form like (\ref{vvcool}) one should already replace the roles of particles and strings for certain types of nodes as we discuss in section \ref{sec:stringhyp}.
%
%For typical representations the weight associated with this element of the Cartan subalgebra is a continuous parameter of the representation. In contrast, the other weights acquire discrete values.
%
%
%
%
%
%Finally, the tensor product of irreps is not necessarily a sum of irreps. This leads to significant complications in the construction of a physical theory \cite{Saleur:2006tf}.
%
%Therefore we see that apart straightforward generalization, the physical theories based on the supersymmetry are more involved then those for the nonsupersymmetric case. A more complete investigation still should be done.
%
%In this chapter we aim to develop techniques mostly for further applications for a thermodynamic Bethe Ansatz (TBA) in the context of the AdS/CFT correspondence. First on the example of $sl(2|1)$ algebra we will recall basic properties of the supersymmetric algebras and theirs representations. Then we will discuss the structure of the representations that appear as a result of the fusion procedure. We will see that, as in the ordinary case, the string-like solutions are in the one-to-one correspondence with rectangular irreps. The corresponding integral equations will be naturally written on a fat hook shape, or in a more general case - on a T-hook shape.
%
\section{\label{sec:sl21algebra}$Sl(2|1)$ algebra and its representations}
%The $sl(2|1)$ algebra is one of the most simples examples of lie superalgebras. In this section we will consider the representation theory of this algebra in details\footnote{Initially the representation theory of this algebra was considered in}. The generalization to the case of $gl(N|M)$ algebra will be given in the next section.

The defining representation of the algebra is given by the following $3\times 3$ matrices
\begin{small}
\be
  e=\left(
      \begin{array}{ccc}
        0 & 1 & 0 \\
        0 & 0 & 0 \\
        0 & 0 & 0 \\
      \end{array}
    \right)\!,\ f=\left(
      \begin{array}{ccc}
        0 & 0 & 0 \\
        1 & 0 & 0 \\
        0 & 0 & 0 \\
      \end{array}
    \right)\!,\ h=\left(
      \begin{array}{ccc}
        1/2 & 0 & 0 \\
        0 & -1/2 & 0 \\
        0 & 0 & 0 \\
      \end{array}\right)\!,\
      B=\left(\begin{array}{ccc}
        1/2 & 0 & 0 \\
        0 & 1/2 & 0 \\
        0 & 0 & 1 \\
      \end{array}\right)\!,&& \no\\
      Q_+=\left(\begin{array}{ccc}
        0 & 0 & 1 \\
        0 & 0 & 0 \\
        0 & 0 & 0 \\
      \end{array}
    \right)\!,\
    Q_-=\left(\begin{array}{ccc}
        0 & 0 & 0 \\
        0 & 0 & 1 \\
        0 & 0 & 0 \\
      \end{array}
    \right)\!,\ S_+=\left(\begin{array}{ccc}
        0 & 0 & 0 \\
        0 & 0 & 0 \\
        0 & -1 & 0 \\
      \end{array}
    \right)\!,\ S_-=\left(\begin{array}{ccc}
        0 & 0 & 0 \\
        0 & 0 & 0 \\
        1 & 0 & 0 \\
      \end{array}
    \right)\!.\hspace{1EM}&&
\ee
\end{small}
\noindent The generators $e,f,h$ of $sl(2)$ bosonic subalgebra obey canonical commutation relations
\be
  [h,e]=e,\ \ [h,f]=-f,\ \ [e,f]=2h.
\ee
The fermionic generators $S_\pm$ and $Q_\pm$ transform under adjoint action of $e,f,h$ as a spin $1/2$ representation. Nonzero commutators are given by
\be
  [h,Q_\pm]&=&\pm\frac 12 Q_\pm,\ \ [h,S_\pm]=\pm\frac 12 S_\pm,\no\\ \
  [e,Q_-]&=&Q_+,\ \ [f,Q_+]=Q_-,\no\\ \
  [e,S_-]&=&S_+,\ \ [f,S_+]=S_-.
\ee

The Cartan subalgebra of $sl(2|1)$ is spanned by $h$ and $B$. The generator $B$ acts as zero on the  bosonic generators. On the fermionic generators it acts as follows
\be
  [B,S_\pm]=\frac 12S_\pm, \ \ [B,Q_\pm]=-\frac 12 Q_\pm.
\ee
%\newpage
%\begin{wrapfigure}{l}{0.5\textwidth}
% \vspace{-12pt}
%  \begin{center}
%    \includegraphics[width=0.35\textwidth]{weightSL21}
%  \end{center}
%  \vspace{-10pt}
%\caption{\label{fig:weightSL21}The weight diagram for the generators of $sl(2|1)$ algebra.}
%\end{wrapfigure}
Finally, the fermionic commutators\footnote{For the case of superalgebras we understand any commutator as a graded commutator, that is anticommutator when both generators are fermionic and usual commutator otherwise.} are given by
\be\label{sl21commutrelations}
  [S_+,Q_+]=-e,\ \ [S_-,Q_-]=f,\ \
  \[Q_\pm,S_\mp\]= h\pm B.
\ee

The weight diagram for the generators is shown in Fig.~\ref{fig:weightSL21}.

\begin{figure}[t]
\centering
\includegraphics[height=6cm]{weightSL21}\qquad
\includegraphics[height=6cm]{irrepSL21}

\parbox[t]{0.45\textwidth}{\caption{\label{fig:weightSL21}The weight diagram for the generators of $sl(2|1)$ algebra.}}\qquad
\parbox[t]{0.45\textwidth}{\caption{\label{fig:irrepSL21}Irreducible representations of $sl(2|1)$. The right one - typical irrep $\langle s,b\rangle$ , the left one - atypical irrep $|s',s'\rangle$. }}
\end{figure}
A standard method to build an irreducible representation of the $sl(2|1)$ algebra is to introduce the highest weight vector $|s,b\rangle$ defined by
\be
  S_+|s,b\rangle =0,\ \ Q_+|s,b\rangle=0,\ \ e|s,b\rangle=0,\ \
  B|s,b\rangle = b|s,b\rangle,\ \ h|s,b\rangle=s|s,b\rangle.
\ee
The other states of the representation are obtained by action of lowering operators $Q_-,S_-$, and $f$. Due to the fermionic nature of $Q_-$ and $S_-$, each of these operators is applied consecutively at most once. For the case when they applied exactly once, we get a typical representation, which we will denote as $\langle s,b\rangle$. Under the action of the bosonic $su(2)\oplus u(1)$ subalgebra this representation decomposes into four $su(2)$ irreps: ($s$,$b$), ($s-1/2,b+1/2$), ($s-1/2,b-1/2$), ($s-1,b$), where the first argument in the brackets is the spin of the $su(2)$ irrep and the second argument is the eigenvalue of the operator $B$. The dimension of $\langle s,b\rangle$ is the following:
\be
  {\rm dim}\langle s,b\rangle=8s.
\ee
The parameter $b$ can acquire arbitrary values except $\pm s$.

An atypical representation is the representation for which either $Q_-|s,b\rangle =0$ or $S_-|s,b\rangle=0$. Due to the commutation relations (\ref{sl21commutrelations}) the first condition can be realized only for $b=s$. The second condition can be realized only for $b=-s$. Both conditions are satisfied simultaneously only when $b=s=0$, \textit{i.e.} for the trivial representation. We will denote the atypical representation with $b=s$  as $|s\rangle$ and the atypical representation with $b=-s$ as $\langle s|$. The reason for such notation is clear from the structure of the representation shown in Fig.~\ref{fig:irrepSL21}. The dimension of atypical represantion is given by
\be
  {\rm dim}|s\rangle={\rm dim}\langle s|=4s+1.
\ee
Since the dimension of atypical representation is smaller then the dimension of typical representation with the same spin, atypical representation is often called short representation.

For $s=1/2$ we have ${\rm dim}|1/2\rangle=3$. This is nothing but the fundamental representation.

The structure of reducible but indecomposable representations is quite involved. Here we would like to point out only the simplest type of indecomposable representation which can be obtained as continuation of the typical representation $\langle b,s\rangle$ to the point $b=s$ (or $b=-s$). The irreducible submodule in such representation is $|s-1/2\rangle$ ($\langle s-1/2|$). %Other types of indecomposable representations do not appear in the fusion procedure which we are going to study. Therefore we do not discuss them here.
For more information about indecomposable representations we refer to \cite{Gotz:2005jz}.
%\begin{figure}[t]
%\centering
%\includegraphics[height=6cm]{irrepSL21}
%\caption{\label{fig:irrepSL21}Irreducible representations of sl(2|1). The right one - typical irrep $\langle s,b\rangle$ , the left one - atypical irrep $|s',s'\rangle$. }
%\end{figure}

It is instructive to identify irreps with the Young tableaux. There are two $3$-dimensional representations: $|1/2\rangle$ and $\langle 1/2|$. We will refer to the first one as fundamental ($3$) and to the second one as antifundamental ($\overline 3$). Following \cite{Balantekin:1980pp}, we label $3$ with a box and $\overline 3$ with a dotted box (see Fig.~\ref{fig:YoungSL21left}). In general, to obtain all irreps one should consider tensor products of $3$ and $\overline 3$. A general irrep corresponds to a union of two Young tableaux \cite{Balantekin:1980pp} shown in Fig.~\ref{fig:YoungSL21left}. It is tempting to answer the question whether it is meaningful to fit this union into the T-hook domain that is introduced in section \ref{sec:Thook}.

An important difference with the $gl(n)$ case is that the antifundamental representation never appears in the tensor product of the fundamental representations. This is also true for a trivial representation, atypical representations with negative $b$ and any typical representations with $b<s$. A natural way to construct antiferromagnetic vacuum is to consider a spin chain with half of the nodes in the fundamental and half of the nodes in the antifundamental representations \cite{Essler:2005ag}. Since tensor products of $3$ and $\overline 3$ contain also indecomposable representations, we will encounter these representations when delaing with the excitations over the antiferromagnetic vacuum.

In the follwing we will consider a simpler particular case - the representations with $b\geq s$.
These representations can be obtained from the tensor product of fundamental representations only.
The tensor product of these representations always decomposes into irreps.
\begin{figure}[t]
\centering
\includegraphics[height=4.5cm]{YoungSL21left}\qquad\qquad\qquad\qquad
\includegraphics[height=4.5cm]{YoungSL21}

\parbox[t]{0.46\textwidth}{\caption{\label{fig:YoungSL21left}At top: fundamental and antifundamental representations. At bottom: an example \cite{Balantekin:1980pp} of irrep that is built from tensor products of fundamental and antifundamental representations.}}\ \ \ \
\parbox[t]{0.46\textwidth}{\caption{\label{fig:YoungSL21}Irreducible representations of $sl(2|1)$ built from tensoring of fundamental representation. At top: atypical irrep $|s'\rangle$, at bottom - typical irrep $\langle s,b\rangle$.}}
\end{figure}

To fix grading of the representation module, we take the vector space with two bosonic and one fermionic components for the fundamental representation. A straightforward combinatorial analysis gives the identification of Young tableaux and irreps shown in Fig.~\ref{fig:YoungSL21}. We used inverse notation for Young tableaux with the largest line below. Such notation was used in \cite{Kazakov:2007fy} to describe Hirota dynamics in integrable systems. Horizontal lines in the Young table mean supersymmetrization: symmetrization of bosonic elements with other elements and antisymmetrization of fermionic elements. The vertical lines in the Young table imply superantisymmetrization: antisymmetrization of bosonic elements with other elements and symmetrization of fermionic elements. Note that Young tableaux give typical irreps only with discrete half-integer values of $b$.

\section{Fusion procedure in the $gl(N|M)$ case.}
The procedure of construction of irreps of $gl(N|M)$ algebra is a straightforward generalization of such procedure for $gl(2|1)$ case. Again, we have a  fundamental representation defined by Dynkin labels $[100\ldots]$ and its conjugate. Arbitrary irrep can be obtained only from tensor product of both of these representations. Appearance of the reducible indecomposable representations in the tensor product is controlled by the value of the continuous parameter $b$. The parameter $b$ is a Cartan weight with respect to the generator $B$, where generator $B$ is given by the following matrix in the defining representation:
\be
  B=\left(
    \begin{array}{c|c}
      N^{-1} \mI_N& 0 \\
      \hline \\
      0 & M^{-1} \mI_M
    \end{array}
  \right)\!.
\ee

In the following we consider only the representations that can be obtained from the tensor product only of the fundamental representation $[100\ldots]$ itself. Such irreps are described by Young tableaux which should be inside a fat hook structure shown in Fig.~\ref{fig:susyhirota}. If the border of a Young table does not touch the internal border\footnote{By the internal border of fat hook we mean the border which contains the corner point $\{M,N\}$.} of the fat hook then such Young table defines atypical representation. Otherwise, such Young table defines typical representation.

We can derive the Hirota dynamics on a fat hook using a straightforward generalisation of discussion in Sec.~\ref{sec:Fusion procedure} \cite{Kazakov:2007fy}. Namely, we consider an integrable system based on the $R$-matrix
\be
  R=\theta-i\scP,
\ee
where $\scP$ is the graded permutation.

Starting with this $R$-matrix one can construct the transfer matrix in a fundamental representation and use a fusion procedure to obtain the transfer matrices in other representations. The transfer-matrices $T^{a,s}[\theta]$ in the rectangular irrep satisfy the Hirota equation
\be
  T^{a,s}\[\theta+\frac i2\]T^{a,s}\[\theta-\frac i2\]=T^{a,s+1}[\theta]T^{a,s-1}[\theta]+T^{a+1,s}[\theta]T^{a-1,s}[\theta].
\ee
The transfer-matrices are non-zero if $a=0$ or $(a,s)$ is inside or on the border of the shape (fat hook) in Fig.~\ref{fig:susyhirota}.

  The representations are nontrivial on the internal border of the fat hook. They are different from the representation in the corner $\{M,N\}$ only by the value of the parameter $b$.


\section{\label{sec:Thook}Bethe Ansatz}

\paragraph{Fat hook case}
\begin{figure}[t]
\centering
\includegraphics[height=5cm]{susyhirota}
\caption{\label{fig:susyhirota}On the left: fat hook for $gl(N|M)$ algebra. On the right: functional equations on $T$ and $F$ for BT2 transform.}
\end{figure}

We will first consider a fat hook configuration. The Bethe Ansatz equations can be derived from the fusion relations via a chain composed from two different types of Backlund transforms. The two different types of Backlund transforms appear in the following way. The bilinear equations (\ref{Backlund}) on $T$ and $F$ considered for a fat hook configuration allow two solutions. For the first one $F$ is nonzero on a fat hook $(N-1,M)$. This is the same Backlund transform which was discussed previously. It is called the Backlund transform of the first type (BT1).

For the second solution  $F$ is nonzero on a fat hook $(N,M+1)$. Exchanging the roles of $T$ and $F$ for such Backlund transform we obtain the Backlund transform of the second type (BT2) which reduces $M$ by one. The functional equations for BT2 are shown in Fig.~\ref{fig:susyhirota}.

%The results of the previous section are directly generalized \cite{Kazakov:2007fy} to the case of the rational $R$-matrix for the $GL(N|M)$ groups. The $R$-matrix of the fundamental particles is given again by (\ref{R-matrix}), where $\CP$ should be understood now as a graded permutation. Hirota equation (\ref{fusioncomplete}) has the same form and is defined on a fat hook shape, depicted on the figure (\ref
%{fig:susyhirota}). There are two possible Backlund transformations. The Backlund transform of the first type (BT1) reduces the fat hook to the one of $GL(N-1|M)$ group. The $T$-$F$ linear system associated with BT1 is the same as in the previous section. The  Backlund transform of the second type (BT2) reduces the fat hook to the one of $GL(N|M-1)$. The associated $T$-$F$ linear system is obtained from that for BT1 by interchanging $T$ and $F$.

The set of the Bethe Ansatz equations is obtained after successive application of Backlund transforms that reduce the fat hook to a single strip. This can be done by application of different chains of Backlund transforms \cite{Kazakov:2007fy}. A possible chain is shown in Fig.~\ref{fig:susyhirota}. The shape of the chain corresponds to a particular Kac-Dynkin diagram of the $gl(N|M)$ algebra. Each turning of the path corresponds to the fermionic node. Each straight pass corresponds to the bosonic node.

The Bethe Ansatz equations are determined by the Cartan matrix of a given Kac-Dynkin diagram and have the formal expression
\be\label{susyBAE}
  \frac{\l_a+\frac i2\delta_{a,1}}{\l_a-\frac i2\delta_{a,1}}=-\prod_{\l_b}\frac{\l_a-\l_b+\frac i2 c_{ab}}{\l_a-\l_b-\frac i2 c_{ab}}.
\ee
The Cartan matrix $c_{ab}$ for a given Kac-Dynikin diagram up to an overall sign is given by the following identification:
\begin{figure}[!h]
\centering
\includegraphics[height=1.5cm]{CartanforDynkin}
%\label{fig:susyhirota}
%\caption{On the left: fat hook for $GL(N|M)$ group. On the right: functional equations on $T$ and $F$ for BT2 transform.}
\end{figure}

The overall sign is chosen such that the sum of the elements in the first row of $c_{ab}$ to be positive.

For example, the Cartan matrix for the Kac-Dynkin diagram in Fig.~\ref{fig:susyhirota} is the following
$$
\left(
  \begin{array}{cccccc}
    2 & -1 & 0 & 0 & 0 & 0 \\
    -1 & 0 & 1 & 0 & 0 & 0 \\
    0 & 1 & -2 & 1 & 0 & 0 \\
    0 & 0 & 1 & 0 & -1 & 0 \\
    0 & 0 & 0 & -1 & 2 & -1 \\
    0 & 0 & 0 & 0 & -1 & 0 \\
  \end{array}
\right).
$$

The Bethe equations (\ref{susyBAE}) can be also written for an arbitrary representation \cite{Ragoucy:2007kg}. It is not clear how to obtain the Bethe equations for an arbitrary representation from a fat hook construction.

\paragraph{T-hook case}

The fat hook construction is well adapted only for the fundamental representations with Dynkin lables $[100\ldots]$. The Bethe Ansatz for other fundamental representations can be obtained if we consider the Hirota system on a so called T-hook shape \cite{Hegedus:2009ky} shown in Fig.~\ref{fig:thook}.

For a T-hook structure two new types of Backlund transforms are possible ($\overline{\rm BT1}$ and $\overline{\rm BT2}$). They reduce the T-hook at the left corner. The functional equations for $\overline{\rm BT1}$ and $\overline{\rm BT2}$ are obtained by mirror reflection of those for BT1 and BT2. Application of all four Backlund transforms finally reduce T-hook to a trivial one. The resulting Bethe equation are written by
\be
   \frac{\l_a+\frac i2\delta_{a,k}}{\l_a-\frac i2\delta_{a,k}}=-\prod_{\l_b}\frac{\l_a-\l_b+\frac i2 c_{ab}}{\l_a-\l_b-\frac i2 c_{ab}}
\ee
The Cartan matrix $c_{ab}$ depends on the path chosen for the reduction of a T-hook. The overall sign of $c_{ab}$ is defined in such a way that $c_{kk}=2$ if $k-th$ node is bosonic and momentum-carrying and we use BT2 or $\overline{\rm BT2}$ as the last step of the chain of Backlund transforms\footnote{Central node on the  left diagram in Fig.\ref{fig:cnodenoncompact} is an example of such node.}. The sign of $c_{ab}$ for other cases follows from duality transformations discussed below.

Note that the T-hook construction for $N=\overline{N}=0$ leads to the Bethe equations for $su(M+\overline{M})$ spin chain in $k$-th antisymmetric representation.

The T-hook structure was first proposed in \cite{Gromov:2009tv}. It was obtained from a string hypothesis that we will discuss below. The relation between the T-hook construction and the representation theory is still not clear.

\begin{figure}[t]
\centering
\includegraphics[height=6cm]{thook}
\caption{\label{fig:thook}T-hook construction. Hirota system defined on a shown domain gives a set of Bethe ansatz equations via a chain of Backlund transforms. The momentum carrying node is shown on the picture.}
\end{figure}


\section{\label{sec:DualityTransformation}Duality transformations.}
The form of the Bethe equations is different depending on what underlying Kac-Dynkin diagram was chosen. Of course these equations should be equivalent. Indeed, there exists a so called duality transformation \cite{GohmannSeel} which allows to pass from one system of equations to another.

Let us consider a fermionic node. We will denote the Baxter polynomial for this node as $Q=\prod (\theta-\theta_k)$. The fermionic node is coupled to two other nodes. We will denote the Baxter polynomials that correspond to these nodes as
\be
  Q_u=\prod (\theta-u_k),\ \ Q_v=\prod (\theta-v_k).
\ee
The Bethe equation for the fermionic node
\be\label{BAEf}
  1=-\frac{Q_u[\theta_k+\frac i2]}{Q_u[\theta_k-\frac i2]}\frac{Q_v[\theta_k-\frac i2]}{Q_v[\theta_k+\frac i2]}
\ee
can be derived from the Baxter equation
\be\label{Bf}
  Q_u^+Q_v^-+Q_u^-Q_v^+=QQ^*.
\ee
From the point of view of a fat hook picture the Baxter polynomials $Q_u,Q_v,Q,Q^*$ are just some $Q_{N'|M'}$ polynomials\footnote{$Q_{N'|M'}$ is the polynomial that defines a boundary condition for the $(N',M')$ fat hook. This is a generalization of the $Q_N$ polynomial in Sec.~\ref{sec:nestedBABacklund}. The polynomial $Q_{N|M}$ gives a source term for the Bethe equations. For the homogeneous spin chain of length $L$ we have $Q_{N|M}=(\theta-\frac i2)^L$.} with appropriate shifts of the arguments on $i/2$. These polynomials are associated to the nodes which form a square shown in Fig.~\ref{fig:duality}. The Baxter equation (\ref{Bf}) is a $QQ$ relation on these polynomials.

\begin{figure}[t]
\centering
\includegraphics[height=3cm]{duality}
\caption{\label{fig:duality}Duality transformation. The nodes denoted by gray can be of any statistics. Obviously, the duality transformation changes the statistics of these nodes.}
\end{figure}


Duality transformation is a passage from the Bethe equations which contain $\theta_k$ as Bethe roots to the Bethe equations which contain $\theta_k^*$ (zeroes of $Q^*$) as Bethe roots. We see that $Q$ and $Q^*$ enter (\ref{Bf}) in a symmetric way. Therefore $\theta_k^*$ are also fermionic roots. They obey the same equation as (\ref{BAEf}), with $\theta_k$ replaced by $\theta_k^*$.

The roots $\theta_j$ enter to the Bethe equations for $u_k$ as the following ratio
\be
  \frac{Q\[u_k-\frac i2\]}{Q\[u_k+\frac i2\]}.
\ee
An analogous ratio appears in the Bethe equations for $v_k$.

Using (\ref{Bf}) it is easy to see that
\be
  \frac{Q\[u_k-\frac i2\]}{Q\[u_k+\frac i2\]}=\frac{Q_u\[u_k-i\]}{Q_u\[u_k+i\]}\frac{Q^*\[u_k+\frac i2\]}{Q^*\[u_k-\frac i2\]}.
\ee
Therefore the Bethe equations for $u_k$ ($v_k$) change in accordance with the change of the Kac-Dynkin diagram shown in Fig.~\ref{fig:duality}.

A special attention should be devoted to the momentum carrying node of a T-hook. If it is fermionic, the Bethe equations for this node are written as
\be
  \(\frac{\theta_k+\frac i2}{\theta_k-\frac i2}\)^L=-\frac{Q_u\[\theta_k+\frac i2\]}{Q_u\[\theta_k-\frac i2\]}\frac{Q_v\[\theta_k-\frac i2\]}{Q_v\[\theta_k+\frac i2\]}.
\ee
The Bethe roots $u_k$ belong to the right wing of the T-hook and the Bethe roots $v_k$ - to the left wing.

If we perform a duality transformation for the momentum carrying node then the building block of the Bethe equations for $v_k$ roots will be the following:
\be
  \frac{Q\[v_k-\frac i2\]}{Q\[v_k+\frac i2\]}=\(\frac{\theta_k-i}{\theta_k+i}\)^L\frac{Q_v\[v_k-i\]}{Q_v\[v_k+i\]}\frac{Q^*\[v_k+\frac i2\]}{Q^*\[v_k-\frac i2\]}.
\ee
Therefore the $v_k$ node becomes also momentum carrying. Although such duality transformation is possible, the resulting equations does not fit into a T-hook construction. Due to this we should forbid to perform the duality transformation of the momentum-carrying node if it is situated inside the Kac-Dynkin diagram. This restriction has interesting consequences. For example, if each wing of the T-hook contains at least one fermionic node, one cannot rewrite the Bethe equations in a form which corresponds to the distinguished diagram (that with a single fermionic node).

The momentum-carrying node in the T-hook construction has another important feature. If we start from the Bethe equations
\be\label{cncomp}
  \(\frac{\theta_k+\frac i2}{\theta_k-\frac i2}\)^L=-\frac{Q\[\theta_k+i\]}{Q\[\theta_k-i\]}\frac{Q_u\[\theta_k-\frac i2\]}{Q_u\[\theta_k+\frac i2\]}\frac{Q_v\[\theta_k-\frac i2\]}{Q_v\[\theta_k+\frac i2\]},
\ee
which correspond to the left diagram in Fig.~\ref{fig:cnodenoncompact}, and perform duality transform both on $u$ and $v$ nodes, then the Bethe equations for the momentum carrying node will become
\be\label{cnnoncomp}
  \(\frac{\theta_k+\frac i2}{\theta_k-\frac i2}\)^L=-\frac{Q\[\theta_k-i\]}{Q\[\theta_k+i\]}\frac{Q_u^*\[\theta_k+\frac i2\]}{Q_u^*\[\theta_k-\frac i2\]}\frac{Q_v^*\[\theta_k+\frac i2\]}{Q_v^*\[\theta_k-\frac i2\]}.
\ee
If we put $Q_u=1$ and $Q_v=1$ in equation (\ref{cncomp}) then we will get the equation for a compact (SU(2)) XXX spin chain. On the opposite, if we put  $Q_u^*=1$ and $Q_v^*=1$ in (\ref{cnnoncomp}) then we will get the equation for a noncompact (Sl(2)) XXX spin chain.

The second description reveals noncompactness of such spin chain. Indeed, let us find the constraints on the possible number of the Bethe roots. For simplicity we suppose that there are only three types of the Bethe roots. Bosonic Bethe roots $\theta_k$ which satisfy (\ref{cncomp}) (or, equivalently (\ref{cnnoncomp})) and fermionic Bethe roots $u_k,v_k$ which satisfy the Baxter equations
\be
  Q^++Q^-=Q_uQ_u^*,\ \ \ Q^++Q^-=Q_vQ_v^*.
\ee
From the Baxter equation we read that
\be\label{numberuv}
  n_\theta=n_u+n_u^*=n_v+n_v^*.
\ee

In Sec.~\ref{sec:countingBethe} we obtained the constraints on the number of bosonic Bethe roots. In our case we have
\be\label{numbertheta}
  n_\theta\leq \frac{L+n_u+n_v}2
\ee
Combining (\ref{numberuv}) and (\ref{numbertheta}) we see that the number of the Bethe roots is unconstrained.

\begin{figure}[t]
\centering
\includegraphics[height=2.5cm]{cnodenoncompact}
\caption{\label{fig:cnodenoncompact}Duality transformation which reveals noncompactness of a T-hook spin chain.}
\end{figure}

\section{\label{sec:stringhyp}String hypothesis and integral equations}
To formulate a set of integral equations in the thermodynamic limit we will establish first the string hypothesis for the Bethe Ansatz based on the $gl(N|M)$ algebra.

The string hypothesis for bosonic roots was discussed in Sec.~\ref{sec:countingBethe} and in Sec.~\ref{sec:PCFGNbound}. Bosonic Bethe roots can form string configurations alone. Also they can participate in the formation of stacks as intermediate nodes. The mechanism how the bosonic roots enter the stacks was discussed in Sec.~\ref{sec:PCFGNbound} in the context of GN and PCF models.

To formulate a string hypothesis for fermionic roots we will consider the Baxter equation for fermionic roots
\be\label{Bf2}
  Q_u[\theta+i/2]Q_v[\theta-i/2]+Q_u[\theta-i/2]Q_v[\theta+i/2]=Q[\theta]Q^*[\theta],
\ee
where the notation is the same as for (\ref{Bf}).

Let us assume for simplicity the following ordering of Bethe roots: $n_u\geq n_\theta\geq n_v$. Then in the thermodynamic limit the roots of $u$ type will determine the dominant term in the l.h.s of (\ref{Bf2}). For ${\rm Im}[u]>0$ the first term will be dominant.

Fermionic Bethe roots do not form string configurations themselves. Instead, they participate in the formation of stacks as the first or the final node. Indeed, if $\theta$-roots organize in a string of length $k$ then (\ref{Bf2}) implies the string configuration with the same center either for $u$-roots of length $k+1$, or for $v$-roots of length $k-1$.

All possible string/stack configurations that can be built from bosonic and fermionic nodes\footnote{For the rational Bethe Ansatz in any fundamental representation.} are shown in Fig.~\ref{fig:stringstacks}
\begin{figure}[!h]
\centering
\includegraphics[height=4cm]{stringstacks}
\caption{\label{fig:stringstacks}Possible string/stack configurations. A) an $s$- string of arbitrary length formed of bosonic roots of the same type. B) an $s$-stack with the longest string of length $s$ formed of fermionic roots. All the other roots are bosonic. The total number of root types is $s$. This stack should terminate with a string of length 1. C) an $(s+k-1)$-stack with the first and the last nodes being fermionic. All other nodes are bosonic. The length of the initiating string is arbitrary.\newline\ \ \
All the centers of strings are situated at the same position. They are depicted in different positions for convenience.\newline\hspace{1EM}
The ordering of number of Bethe roots in the nested Bethe Ansatz is the following: the node with the largest amount of roots is on the left.}
\end{figure}

\subsubsection{Integral equations on a fat hook}
The procedure of construction of integral equations is analogous to the one described for the bosonic case. In appendix \ref{app:susy} we prove the following statement:

The set of the functional equations derived from the Bethe Ansatz for a given Kac-Dynkin diagram of $gl(N|M)$ algebra and under the assumption that the string hypothesis is valid is equivalent to the following set of equations:
\be\label{fathookie}
  \delta_{a,1}\delta_{s,1}R_p=\sum_{a'}C_{aa'}R_{a',s}+\sum_{s'}C_{ss'}\overline{R}_{a,s'},
\ee
for $\{a,s\}$ being a coordinate of a point situated strictly inside the fat hook, and
\be\label{TMN}
  R_{M,N}+{\overline R}_{M,N}=T_{M,N}
\ee
for $a=N, b=M$, where $T_{M,N}$ is different for different Kac-Dynkin diagrams; the expression for of $T_{M,N}$ is given in (\ref{TNM1}) and (\ref{TNM2}).

$C_{aa'}$ is a "D-deformed" Cartan matrix defined by
\be\label{cddcdd}
  C_{aa'}=(D+D^{-1})\delta_{aa'}-\delta_{a,a'+1}-\delta_{a,a'-1}.
\ee
The resolvents $R_{a,s}$ and ${\overline R}_{a,s}$ are zero on the boundary and outside the fat hook except for $R_{N,M}, \overline{R}_{N,M}$.

There is a string configuration associated with each $\{a,s\}$ node of a fat hook. Depending on the node, either $R_{a,s}$ or ${\overline R}_{a,s}$ is the resolvent of the density function of strings. Then correspondingly
either ${\overline R}_{a,s}$ or $R_{a,s}$ is the resolvent of the correspondent density of holes.
\begin{figure}[t]
\centering
\includegraphics[height=6cm]{stringfathook}
\caption{\label{fig:stringfathook}Organization of strings into fat hook. The blue line shows the path of embedding of the Kac-Dynkin diagram. Green lines show the string configurations based on the bosonic nodes. Red lines show stack configurations based on the fermionic nodes.}
\end{figure}

The exact identification of $R_{a,s}$ with holes or particles is given by the following procedure. First we draw the Kac-Dynkin diagram on the nodes of the fat hook. The momentum-carrying node corresponds to the node \{1,1\}. We are allowed then to move only to the east or to the north. The initial direction is to the east(north) if the last movement in the chain of the Backlund transforms was to the west(south). For example for the fat hook construction in Fig.~\ref{fig:susyhirota} the initial direction is to the north.

One should turn at each node next to the fermionic one. %If the movement was done correctly then the last node of the Kac-Dynkin diagram should be at the position $\{N,M\}$.

Each node of the fat hook occupied by the Kac-Dynkin diagram is associated with the corresponding type of the Bethe roots. The string/stack configurations with the longest string formed from this type of Bethe roots are situated on the straight line which starts from the considered node. There is the only way to assign straight lines to the nodes of the Kac-Dynkin diagram such that all nodes of the fat hook will be occupied.

The example of the whole construction is shown in Fig.~\ref{fig:stringfathook}.

The correspondence between holes/particles and $R/{\overline R}$ is chosen in a such way that interaction (in the sense of equation (\ref{fathookie})) inside the same line should be through the holes and the interaction between different lines should be through the particles.

%The derivation of (\ref{fathookie}) is a little bit technical. We give it in the appendix \ref{app:susy}.

The derivation of (\ref{fathookie}) given in appendix \ref{app:susy} can be easily generalized for the T-hook shape. The equations (\ref{fathookie}) remain the same.

Although formally the equations (\ref{fathookie}) are the same for different Kac-Dynkin diagrams, these equations describe different regimes of a spin chain. As well, in general there is no relations between the resolvents used in (\ref{fathookie}) for different Kac-Dynkin diagrams. We will illustrate now this issue on the example of $sl(2|1)$ spin chain

\section{Thermodynamic limit of the Bethe equations in the $sl(2|1)$ case}
In the $gl(n)$ case we can consider the thermodynamic limit for configurations close either to the ferromagnetic or to the antiferromagnetic vacuum. In the supersymmetric case there are more possibilities.

Let us consider the Bethe equations for $sl(2|1)$ spin chain in a fundamental representation.
Each site of the spin chain is occupied by one particle which can be a boson with spin up or down or a fermion.

From the representation theory we conclude that the number of fermions can be changed only by $\pm 1$ by the action of the symmetry algebra. Indeed, the number of fermions is changed under action of $Q_\pm$ and $S_\pm$ generators. The square of these generators is zero.

Therefore the state with large amount of fermions never lies in the same symmetry multiplet with the state with small amount of fermions. Thus we have four possible regimes in the thermodynamic limit. If we choose as the pseudovacuum a state with each site occupied with bosons with spin down then these regimes are described as follows:
\begin{wrapfigure}{r}{0.45\textwidth}
 %\vspace{-20pt}
  \begin{center}
    \includegraphics[width=0.3\textwidth]{tdlimitSL21}
  \end{center}
  \vspace{-15pt}
  \caption{\label{fig:highestweightvectors}The position of highest weight vectors of the states that correspond to different regimes.}
\end{wrapfigure}
\bn
  \item Large spin, small amount of fermions.
  \item Small spin, small amount of fermions.
  \item Large spin, large amount of fermions.
  \item Small spin, large amount of fermions.
\en
%\newpage
It turns out that different types of the thermodynamic limit, except the second one, are naturally related to different dual configurations of the Bethe equations. We will consider each configuration separately.

\paragraph{}{\bf\xOX case.\hspace{1EM}}
In this case the Bethe equations are written as
\be\label{someBethe2}
  \(\frac{\theta+\frac i2}{\theta-\frac i2}\)^L&=&-\prod_{\theta'}\frac{\theta-\theta'+i}{\theta-\theta'-i}\prod_{u}\frac{\theta-u-\frac i2}{\theta-u+\frac i2},\no\\
  -1&=&\prod_\theta\frac{u-\theta+\frac i2}{u-\theta-\frac i2}.
\ee
The inequalities for the number of Bethe roots are written as follows
\be\label{ineq1}
  n_u\leq n_\theta,\  \ n_\theta\leq\frac{L+n_u}{2}\leq L.
\ee
Naturally, the thermodynamic limit is possible in the case when we replace all inequalities $\leq$ by stronger demands $\ll$. This corresponds to the first type of the thermodynamic limit.

The bosonic Bethe roots $\theta$ can form string configurations while the fermionic roots are real. Introducing the resolvents $R_s$ for the $s$-strings and $F$ for fermions we obtain the integral equations
\be
  \delta_{s,1}R_p&=&C^\infty_{ss'}R_{s'}^*+(D+D^{-1})R_s-\delta_{s,1}F,\no\\
  0&=&D^{s'}R_{s'}-F-F^*
\ee
One can try to perform a particle-hole transformation of $R_1$ as we did in the $su(2)$ case. In this way we will realize the second type of the limit. The obtained integral equations seem do not correspond to the asymptotic Bethe Ansatz of any known integrable field theory.

\paragraph{}{\bf\xXX case.\hspace{1EM}}
This case is obtained from the previous one by performing the dualization of the root $u$. The Bethe equations are written as
\be\label{someBethe1}
  \(\frac{\theta+\frac i2}{\theta-\frac i2}\)^L&=&-\prod_{{u^*}}\frac{\theta-{u^*}+\frac i2}{\theta-{u^*}-\frac i2},\no\\
  -1&=&\prod_\theta\frac{{u^*}-\theta+\frac i2}{{u^*}-\theta-\frac i2}.
\ee
The inequalities for number of Bethe roots are written as follows
\be
  n_{u^*}\leq n_\theta\leq\frac{L}{2},\  \ n_\theta\leq {L-n_{u^*}}.
\ee
The thermodynamic limit corresponds to the case when $n_u\lesssim n_\theta$, which is a third type of thermodynamic limit.

Since the resolvents $R_s$ remain the same as in the previous case, all the integral equations which do not include $F$ should remain the same. This is indeed the case.  Note that the underlying $s$-string configurations in the \xOX case correspond to stack configurations of two fermionic nodes in the \xXX case.

The complete set of integral equations is written as
\be
\delta_{s,1} R_p&=&C^\infty_{ss'}R_{s'}^*+(D+D^{-1})R_s-\delta_{s,1}F_*^*,\no\\
0&=&D^{s'}R_{s'}-F_*-F_*^*,
\ee
where by $F_*$ we denoted the resolvent for dual variables and by $F_*^*$ the resolvent of holes for the dual variables. Note that by construction $F_*^*\neq F$. %Also, the sense (but not the value) of $R_1$ have been changed. $R_1$ now describes fermionic excitations.

\paragraph{}{\bf\xXO case.\hspace{1EM}}
This case is obtained after duality transformation on the $\theta$-variable of the \xXX case. The Bethe equations are written as
\be\label{someBethe1}
  \(\frac{\theta^*+\frac i2}{\theta^*-\frac i2}\)^L&=&-\prod_{{u^*}}\frac{\theta^*-{u^*}+\frac i2}{\theta^*-{u^*}-\frac i2},\no\\
  -1&=&\prod_{{u^*}'}\frac{{u^*}-{u^*}'+i}{{u^*}-{u^*}'-i}\prod_\theta^*\frac{{u^*}-\theta^*-\frac i2}{{u^*}-\theta^*+\frac i2}.
\ee
This case is the best suited for description of the low-spin regime with most of the excitations being fermions (case 4). The $s$-string of $\theta$-s in the \xOX case transforms into $s-1$ string of $u^*$-s in the \xXO case. The bosonic excitations of the \xOX case are now described by the stack composed of $\theta^*$ 2-string and one $u^*$ Bethe root. We will denote the resolvent of $s-1$-string configuration, $s\geq 2$, by $R_s$ (it should be the same resolvents as in previous case), the resolvent for free $\theta^*$ roots by $R_1$, and the resolvent for the stack by $G$.
Then the integral equations will be written as
\be
  \delta_{s,1} R_p&=&C^\infty_{ss'}R_{s'}^*+(D+D^{-1})R_s-\delta_{s,1}G^*,\no\\
0&=&\sum_{s'=2}^\infty D^{s'}R_{s'}-D R_1^*-G-G^*.
\ee

\begin{figure}[t]
\centering
\includegraphics[height=3cm]{tdsl21}
\caption{\label{fig:tdsl21}Organization of integral equations for different Kac-Dynkin diagrams of $sl(2|1)$.}
\end{figure}

\section{T-hook}
In the previous two chapters we discussed an algebraic structure of the functional equations for the case of the irrep $[100\ldots]$ of the $gl(N|M)$ algebra. This structure has a natural generalization for the case of other fundamental representation. Let us consider an integrable system which is described by the following Kac-Dynkin diagram:
\be\label{KDinside}
    \parbox[c]{6.1cm}{\includegraphics[width=6cm]{Dynkinglnmglnm}}.
\ee
This is a diagram of the $gl(N+N'|M+M')$ algebra\footnote{If a grading convention is not specified, it could be also $gl(N+M'|M+N')$ algebra. However, we can always define a self consistent notation to obtain only $gl(N+N'|M+M')$ case}.  Gray nodes stay either for bosonic or fermionic nodes. Therefore we do not require the Kac-Dynkin diagram to be distinguished. Numbers above the nodes are the Dynkin labels of the representation. 

By a direct generalization of the results of (\ref{sec:stringhyp}) we obtain that the interactions between string configurations in the thermodynamic limit of the Bethe Ansatz based on (\ref{KDinside}) are described by (\ref{fathookie}) which is now defined on a $T$-hook shape shown in Fig.~\ref{fig:thook}. 
